Max-Margin Works while Large Margin Fails: Generalization without Uniform Convergence

A major challenge in modern machine learning is theoretically understanding the generalization properties of overparameterized models. Many existing tools rely on uniform convergence (UC), a property that, when it holds, guarantees that the test loss will be close to the training loss, uniformly over a class of candidate models. Nagarajan and Kolter (2019) show that in certain simple linear and neural-network settings, any uniform convergence bound will be vacuous, leaving open the question of how to prove generalization in settings where UC fails. Our main contribution is proving novel generalization bounds in two such settings, one linear, and one non-linear. We study the linear classification setting of Nagarajan and Kolter, and a quadratic ground truth function learned via a two-layer neural network in the non-linear regime. We prove a new type of margin bound showing that above a certain signal-to-noise threshold, any near-max-margin classifier will achieve almost no test loss in these two settings. Our results show that near-max-margin is important: while any model that achieves at least a $(1 - \epsilon)$-fraction of the max-margin generalizes well, a classifier achieving half of the max-margin may fail terribly. Building on the impossibility results of Nagarajan and Kolter, under slightly stronger assumptions, we show that one-sided UC bounds and classical margin bounds will fail on near-max-margin classifiers. Our analysis provides insight on why memorization can coexist with generalization: we show that in this challenging regime where generalization occurs but UC fails, near-max-margin classifiers simultaneously contain some generalizable components and some overfitting components that memorize the data. The presence of the overfitting components is enough to preclude UC, but the near-extremal margin guarantees that sufficient generalizable components are present.

==> sections/abstract.tex <==
\begin{abstract}
A major challenge in modern machine learning is theoretically understanding the generalization properties of overparameterized models. Many existing tools rely on \em uniform convergence \em (UC), a property that, when holds, guarantees that the population loss will be close to the empirical training loss, uniformly over a class of candidate concepts. \citet{nagarajan2019uniform} show theoretically and empirically the failure of any two-sided UC bound to guarantee any generalization for certain overparameterized linear problems and nonlinear problems respectively. Our main results strengthen these impossibility results and prove novel margin-based bounds that can guarantee generalization even when UC fails. We consider two well-studied linear and non-linear binary classification problems: the setting of \citet{nagarajan2019uniform} for the linear problem, and a quadratic ground truth function learned via a two-layer neural network in the non-linear setting. We strengthen the UC impossibility results of \citet{nagarajan2019uniform}, proving that near-max margin classifiers cannot be proven to generalize via one-sided UC bounds or standard margin bounds. Then, we prove via a new type of margin bound showing that any near max-margin classifier will achieve almost no test loss in these two settings. \mg{TODO, implement Tengyu's comments to focus more on margin generalization result, and less on background.}

{\textbf{Take 2}}
In this work, we study the generalizability of near-max-margin classifiers in overparameterized regimes where uniform convergence and classical margin bounds fail. We consider two well-studied linear and non-linear binary classification problems: a high-dimensional linear problem, and a quadratic ground truth function learned via a two-layer neural network in the non-linear setting. Building upon the work of \citet{nagarajan2019uniform}, we prove that below a certain signal-to-noise ratio, any one-sided uniform convergence (UC) bound will be vacuous. Akin to \citet{nagarajan2019uniform}, we only require that such a UC bound be uniform over the set of near-max-margin classifiers output with high probability from samples drawn from the structured distributions above. We prove that above as second \em lower \em signal-to-noise threshold, any near-max-margin classifier generalizes. Our results show that max margin is important --- while a classifier achieving a margin that is $(1 - \epsilon)$-optimal provably generalizes well, a classifier achieving half of the max-margin may fail terribly. Classical margin bounds, which are typically proven via UC, often are continuous in the margin and thus fail to capture this kind of phase transition. Our analysis reveals that in this challenging regime where generalization occurs but UC fails, near-max margin classifiers simultaneously contain some generalizable components and some spurious components that memorize the data. The presence of the spurious components is enough to doom UC, but the near-extremal margin guarantees that sufficient generalizable components are present.\mg{Fix. Main issue is lack of motivation and selling result - see ML Lunch comments.}


{\textbf{Take 3}}
A major challenge in modern machine learning is theoretically understanding the generalization properties of overparameterized models. Many existing tools rely on \em uniform convergence \em (UC), a property that, when holds, guarantees that the population loss will be close to the empirical training loss, uniformly over a class of candidate concepts. \citet{nagarajan2019uniform} show the in certain simple linear and neural-network settings, and uniform convergence bound will be vacuous Our main results strengthen these impossibility results and prove novel margin-based bounds that can guarantee generalization even when UC fails. We consider two well-studied linear and non-linear binary classification problems: the setting of \citet{nagarajan2019uniform} for the linear problem, and a quadratic ground truth function learned via a two-layer neural network in the non-linear setting. We strengthen the UC impossibility results of \citet{nagarajan2019uniform}, proving that near-max margin classifiers cannot be proven to generalize via one-sided UC bounds or classical margin bounds. Then, we prove a new type of margin bound showing that any near max-margin classifier will achieve almost no test loss in these two settings. Our results show that max margin is important --- while a classifier achieving a margin that is $(1 - \epsilon)$-optimal provably generalizes well, a classifier achieving half of the max-margin may fail terribly. Classical margin bounds, which are typically proven via UC, often are continuous in the margin and thus fail to capture this kind of phase transition. Our analysis reveals that in this challenging regime where generalization occurs but UC fails, near-max margin classifiers simultaneously contain some generalizable components and some spurious components that memorize the data. The presence of the spurious components is enough to doom UC, but the near-extremal margin guarantees that sufficient generalizable components are present.

\end{abstract}

==> sections/trivariate.tex <==
\begin{proof}
Because of the homogeneity of each constraint, it suffices to prove the result for $N_4 = 1$. Consider some $\epsilon$-optimal solution $(b, c, d)$. Without loss of generality, by the symmetry of the problem, we can assume $b$ is non-negative. 

Let $\gamma_0$ be the best objective value achieved when $b = 0$, and let $\gamma_{*}$ be the best objective value achieved when $d = 0$.

\begin{claim}
If $d = 0$, the best objective value is found by setting $b = \sqrt{\frac{\kappa}{4 + \kappa}}$ and $c = \sqrt{\frac{16}{(4 + \kappa)\kappa}}$.
\end{claim}

\begin{claim}
For any $b >0, c, d$,
\begin{align}
    \phi(b + c) +  \phi(-b + d) \leq \gamma_0 + 4b
\end{align}
\end{claim}
\begin{proof}
\begin{align}
    \phi(b + c) +  \phi(-b + d) &\leq \phi(b + c) +  \phi(d)\\
    &\leq \phi(c) + \phi(d) + b\sup_{c, d: b^2 + \frac{\kappa}{4} c^2 \leq 1}\sigma^\prime(b + c)\\
    &\leq \phi(c) + \phi(d) + 4b.
\end{align}
Here in the second inequality we used the fact that the derivative of $\sigma$ is increasing, and in the third inequality we used the explicit maximizing solution for $b$ and $c$ from the proof of the previous claim and the fact that $\kappa \geq 1$.

By definition, the maximum feasible value of the last line is $\gamma_0 + 4b$.
\end{proof}
Using this claim, if a solution is $(1 - \epsilon)$-optimal, we must have $\gamma_0 + 4b \geq (1 - \epsilon)\gamma_*$, so $b \geq \frac{(1 - \epsilon)\gamma_* - \gamma_0}{4}$.

Now $\phi(b + c) \leq \gamma_*$, so we have
\begin{align}
    \frac{\phi(b)}{\phi(b + c)} \geq \frac{\phi\left(\frac{(1 - \epsilon)\gamma_* - \gamma_0}{4}\right)}{\gamma_*}.
\end{align}
To prove the second statement, we need to show that $d \leq b$ such that $\phi(-b + d) = 0$.

\todot{There are some parts missing from this proof, that have only been numerically verified on Desmos.}
\end{proof}
